Recurrent Interaction Network for Jointly Extracting Entities and Classifying Relations

The idea of using multi-task learning approaches to address the joint extraction of entity and relation is motivated by the relatedness between the entity recognition task and the relation classification task. Existing methods using multi-task learning techniques to address the problem learn interactions among the two tasks through a shared network, where the shared information is passed into the task-specific networks for prediction. However, such an approach hinders the model from learning explicit interactions between the two tasks to improve the performance on the individual tasks. As a solution, we design a multi-task learning model which we refer to as recurrent interaction network which allows the learning of interactions dynamically, to effectively model task-specific features for classification. Empirical studies on two real-world datasets confirm the superiority of the proposed model.

==> intro.tex <==
\section{Introduction}\label{introduction}
The extraction of entities and relations from textual data comprises of two sub-tasks: entity recognition (ER) and relation classification (RC). The ER task aims to extract all entities in a given text. The RC task aims to classify the relation between any pair of entities in the text. In practice, both tasks are required to be solved jointly, and have been observed to contribute significantly in extracting structured knowledge from unstructured text for several applications, including knowledge base construction~\cite{DBLP:conf/acl/KomninosM17,DBLP:conf/aaai/DengXLYDFLS19,DBLP:conf/acl/NathaniCSK19}. For instance, consider the sentence \emph{John was born in Sheffield, a city in the north of England}. The goal of a joint entity and relation extraction task is to identify all the factual relational triples (or relational facts) \emph{\tt (Sheffield, birth\_place\_of, John)} and \emph{\tt (England, contains, Sheffield)}. %This joint task plays a vital role in extracting structured knowledge from unstructured text, which is deemed important for several applications, including knowledge base construction~\cite{DBLP:conf/acl/KomninosM17,DBLP:conf/aaai/DengXLYDFLS19,DBLP:conf/acl/NathaniCSK19}.  


%Named entity recognition (NER) and relation extraction (RC) are two crucial tasks for information extraction from textual data. NER aims to extract all entities in the sentence. RC aims to classify the relation between given entities.

%In practice, both of two tasks are required to be solved simultaneously. Consider the sentence, \emph{John was born in Sheffield which is a city of England} as an example. The goal of the joint entity and relation extraction is to identify all the relational triples \emph{\tt (Sheffield, birth\_place\_of, John)} and \emph{\tt (England, contains, Sheffield)}. This joint task plays a vital role in extracting structured knowledge from unstructured text, which is deemed important for several applications, including knowledge base construction~\cite{DBLP:conf/acl/KomninosM17,DBLP:conf/aaai/DengXLYDFLS19,DBLP:conf/acl/NathaniCSK19}.

The simplest approach to solve this joint task is to utilize a pipeline-based approach by firstly extracting all entities in the sentence and then classifying the relation between all entity pairs~\cite{DBLP:journals/jmlr/ZelenkoAR03,DBLP:conf/acl/ZhouSZZ05,DBLP:conf/acl/ChanR11}. However, pipeline-based approaches disregard the correlation between ER and RC tasks, leading to error propagation in these methods.


Considering the close correlation between ER and RC tasks, many recent methods have exploited multi-task learning (MTL) techniques~\cite{DBLP:conf/icml/CollobertW08} to capture the correlation between the two tasks~\cite{DBLP:conf/acl/MiwaB16,DBLP:conf/acl/FuLM19,zeng2019copymtl}. MTL-based methods improves the generalization performance of the RC task with the help of the ER task, and vice versa, to improve the performance of each individual task. These are conventional MTL-based methods which employ a shared network to learn interactions between the two tasks, and extract a shared common representation which is exploited by task-specific networks. In a sense, this approach implicitly models the correlation of ER and RC since the task-specific networks have no further control over the learning of interactions. Thus, the previous methods assume that the shared network is sufficient in learning the correlation between the two tasks.

%It is worth noting that MTL-based methods improves the generalization performance of the RC task with the help of the ER task, and vice versa to improve the performance of each individual task.

%via a shared common representation
%Considering the close correlation between ER and RC tasks, many recent studies have been focused on the joint entity and relation extraction task. Multi-task learning (MTL) techniques~\cite{DBLP:conf/icml/CollobertW08} have been exploited to capture the correlation between ER and RC and improve the joint extraction performance~\cite{DBLP:conf/acl/MiwaB16,DBLP:conf/acl/LiuZZHZ18,DBLP:conf/acl/FuLM19}. These MTL-based models implicitly model the correlation of ER and RC via a shared common representation. It is worth noting that MTL-based methods improves the generalization performance of the RC task with the help of the ER task, and vice versa.

%It is worth noting that the output of RC helps the prediction of ER and vice versa.

%\textcolor{red}{Take the sentence \emph{Reynolds had been in CBS for ten years} as an example. If we know that there exist the relation \emph{\tt company\_of} between \emph{CBS} and \emph{Reynolds}, then \emph{CBS} and \emph{Reynolds} have high probabilities to be \emph{\tt Organization} and \emph{\tt Person} while having low probabilities to be \emph{\tt Person} and \emph{\tt Person}. On the other hand, if we know \emph{CBS} and \emph{Reynolds} are \emph{\tt Organization} and \emph{\tt Person}, then the relation is impossible to be \emph{\tt nationality\_of}. In this study, we regard NER and RC as dual tasks and introduce an interaction model between the output of NER and RC to explicitly leverage their correlation to guide the training process of both models.} 

Even so, identifying the relational facts in sentences is a difficult problem. Reason being that several relational facts may overlap in a sentence~\cite{DBLP:conf/emnlp/Zhang0M18}. Although a conventional MTL method~\cite{DBLP:conf/icml/CollobertW08} may learn task-specific features and has been successfully applied in a wide variety of scenarios~\cite{DBLP:conf/ijcai/ZhangW16a,DBLP:conf/emnlp/WuSCHS16,DBLP:conf/naacl/GooGHHCHC18,DBLP:conf/emnlp/HanNP19,DBLP:conf/aclnut/LiBZL19,DBLP:conf/emnlp/NishinoMKTMO19,DBLP:conf/acl/LiuHCG19,DBLP:conf/acl/HuPHLL19}, it is limited in learning implicit interactions between the ER and the RC tasks. These interactions may not sufficiently capture the complex interactions that exist between the two tasks. For that reason, the classifiers for the two individual tasks may be deficient in having a good bias-variance tradeoff. Without modeling explicit interactions, as shown in an aspect-level sentiment classification task \cite{DBLP:conf/acl/HeLND19}, the existing MTL-based methods~\cite{DBLP:conf/acl/MiwaB16,DBLP:conf/acl/FuLM19,zeng2019copymtl} cannot effectively capture the correlation between the ER and the RC tasks.

In this paper, we overcome the aforementioned limitation of previous methods by proposing a recurrent interaction network (RIN) to effectively capture the correlations between the ER and RC tasks. The model can be interpreted as a multi-task architecture which leverages an interaction mechanism as a strategy to explicitly learn the interactions between the ER and RC tasks, with the intention of refining the classifiers of the two tasks. More specifically, the interaction mechanism is a recurrent structure comprising of multiple interaction layers, to progressively learn complex interactions while refining the prediction of the ER and RC tasks. As shown by our experiment such a mechanism progressively provides discriminating features which is an essential requirement for the individual task. Empirical studies on NYT and WebNLG datasets achieve new state-of-the-art performances and confirm the effectiveness of the proposed RIN model.

% \begin{figure}[htbp]
% \centering
% 	\renewcommand\tabcolsep{0pt}
% 	\begin{tabular}{c c}
% 	\scalebox{0.65}{\input{intro1.tex}} &
% 	\scalebox{0.65}{\input{intro2.tex}}
% 	\\
% 	  	(A) &
% 	  (B) 
% 	\end{tabular}
% 	\caption{(A) A generalized multi-task model. (B) An interaction augmented multi-task model. $X$ is the input, $g_1$ and $g_2$ are two models for different tasks. They correspond to ER and RC in this study. The ``$\circ$'' node is a neural network.}
% 	\label{fig:motivation}
% \end{figure}

%\textcolor{red}{As shown in Figure~\ref{fig:motivation}(A), most previous works~\cite{DBLP:conf/acl/MiwaB16,DBLP:conf/acl/LiuZZHZ18,DBLP:conf/acl/FuLM19,zeng-etal-2019-learning,zeng2019copymtl} using a multi-task learning architecture for jointly extracting entities and relations learn shared layers $f$  to extract common features $S$ for the ER and RC tasks. Further, these features are fed to separate task-specific channels $g_1$ and $g_2$ for the respective ER and RC tasks, with the aim to learn task-specific features for classification. If $f$ models sufficient statistics of $X$ for accurately predicting the target $y_1$ and $y_2$, it implies $g_1$ and $g_2$ are sufficiently expressive and the data supports the learning of $g_1$ and $g_2$. However, this is not always the case due to the generalization behaviour of $f$, i.e. the shared features $S$ may not effectively capture the intrinsic interactions existing between the two tasks. To get a satisfactory balance between bias-variance trade-off for $g_1$ and $g_2$, we need to explicitly learn higher-order interactions between $g_1$ and $g_2$ by means of the shared features $S$ as shown in Figure~\ref{fig:motivation}(B). Although a generalized multi-task method may model the implicit interactions between the two tasks, explicitly modeling multiple interactions supports to learn a relatively expressive model. The interaction can be operated for multi rounds. The prediction of the tasks will be progressively refined. We also conduct experiments on the interaction rounds to verify our assumption.}















%As shown in Figure~\ref{fig:motivation} (A), most previous works jointly extracting entities and relations in a multi-task learning framework which focuses on learning share layers $f$ to extract the common features $S$ for NER and RE. Then, the learned common features $S$ are fed into two independent modules $g_1$ and $g_2$ for NER and RE. If $f$ computes the sufficient statistics of $X$ for predicting $y_1$ and $y_2$, $g_1$ and $g_2$ are sufficiently expressive and data supports the learning of $g_1$ and $g_2$, there is no need to have further interaction. However, there is not always the case, especially when $g_1$ and $g_2$ correlates to each other. An interaction between $g_1$ and $g_2$ can be introduced as shown in (B). Although the interactive MTL framework may be less expressive for the simple interaction, multiple interactions allow each component to be less expressive but overall the model is sufficiently expressive.

%Based on this motivation, we propose a recurrent interaction network (RIN) to capture the correlations between the NER and RC tasks. \textcolor{red}{Specifically, we present a method to learn the dual task interaction features which represent the ``degree of alignment'' of NER and RC on each word. We further introduce a recurrent structure to progressively refine the prediction of NER and RC based on the learned dual task interaction features. The empirical studies on NYT and WebNLG datasets achieve new state-of-the-art performances and confirm the effectiveness of the presented RIN. A further experiment by introducing a pre-trained BERT~\cite{DBLP:conf/naacl/DevlinCLT19} model as the sentence encoder shows a significant performance gain over the BiLSTM encoder. This fact suggests the utilizing of BERT in the joint entity and relation extraction tasks.}

% \textcolor{red}{Based on this observation, we propose a recurrent interaction network (RIN) to effectively capture the correlations between the ER and RC tasks. More specifically, we present a method based on Recurrent Neural Networks~\cite{} to learn interaction features which represent the ``degree of alignment'' of ER and RE.  We further introduce a recurrent structure to progressively refine the prediction of NER and RC based on the learned interaction features. Empirical studies on NYT and WebNLG datasets achieve new state-of-the-art performances and confirm the effectiveness of the proposed RIN model. A further experiment exploiting pre-trained BERT~\cite{DBLP:conf/naacl/DevlinCLT19} model as a sentence encoder shows a significant performance gain over the BiLSTM encoder.}



==> relworks.tex <==
% \section{Related Work}\label{relworks}
% Relation extraction is one of the most important tasks in natural language processing. This task aims to extract relational facts from the raw text. In the earlier relation extraction studies, researchers aim to classify the relation between two entities which are given in a sentence. For this relation classification task, existing works mainly fall into two classes: the sequence based models and the dependency based models. 
% The sequence based models only take as input the word sequence of the sentence and employ attention mechanism to distill a representation for the classification task~\cite{DBLP:conf/paclic/ZhangZHY15,DBLP:conf/coling/ShenH16,DBLP:conf/acl/WangCML16}. The dependency based models aim to incorporate dependency information into the neural model for the purpose of enhancing the precision of relation extraction for the given entities in text~\cite{DBLP:conf/emnlp/XuMLCPJ15,DBLP:conf/acl/MiwaB16,DBLP:conf/emnlp/Zhang0M18,DBLP:conf/acl/GuoZL19}. 

% These proposed methods require that entities are already marked in the sentence. More practically, sentences are not accompanied with marked entities. A more challenging task is to extract all relational facts from an arbitrary sentence which are free from marked entities.
% Many researchers have proposed to address this task in a pipeline by firstly extracting all entities in the sentence, then classifying the relation between all entity pairs~\cite{DBLP:journals/jmlr/ZelenkoAR03,DBLP:conf/acl/ZhouSZZ05,DBLP:conf/acl/ChanR11}. However, the pipeline based methods may result in error propagation which hurts the model performance. 
% Some other methods depend on complex manual designed features~\cite{DBLP:conf/acl/LiJ14,DBLP:conf/emnlp/MiwaS14,DBLP:conf/coling/GuptaSA16}.


% Instead of trying to extract all the relational triples in the sentence, \cite{DBLP:conf/acl/ZhengWBHZX17} proposed a tagging strategy to transfer this task into a sequence prediction problem. The label of relation and entity type are shared in a common space. The model is required to classify the entity type and relation simultaneously. However, their method fails to address the cases where more than one relations exist between two entities. \cite{DBLP:conf/emnlp/Zhang0M18} proposed an end-to-end sequence-to-sequence model for jointly extracting entities and relations. Their model detects a relational triple by firstly decoding the relation, then decoding the two entities of the relation. However the number of relational triples which can be extracted in a sentence is limited to a pre-difined constant. Their model can not extract the entities which have multi words either. \cite{DBLP:conf/acl/FuLM19} exploit a Bi-LSTM on the top of graph convolutional network (GCN)~\cite{DBLP:conf/iclr/KipfW17} to both encode the linear and dependency structure of the sentence. Further, they proposed a $2$nd-phrase relation-weighted GCN to further model the interaction between different relations. \cite{DBLP:journals/corr/abs-1909-03227} designed a hierarchical binary tagging framework for joint entities and relations extraction. They further improve the extraction by leveraging the pre-trained BERT~\cite{DBLP:conf/naacl/DevlinCLT19} model to initialize the word embedding. As discussed above, most previous works leverage the MTL framework for jointly detecting entities and classifying relations. They fail to consider the implicit constrain in the two tasks. In this paper, we not only proposed to consider the constrain by explicitly modeling the interaction of the two task, but also introduce the recurrent interaction network to progressively refine the extraction of entities and relations.

% \begin{figure*}[htbp]
% 	\centering
% 	\scalebox{1.}{\input{our_model.tex}}
% 	\caption{Overview of RIN.}
% 	\label{fig:our_model}
% \end{figure*}

\section{Related Work}\label{relworks}
Extracting relational facts from raw text is one of the most important tasks in natural language processing. In the early works proposed for the task, most researchers adopt sequence based models and attention mechanisms to extract a vector representation for classifying relational triples~\cite{DBLP:conf/paclic/ZhangZHY15,DBLP:conf/coling/ShenH16,DBLP:conf/acl/WangCML16}. Some other studies also incorporate the dependency grammar information of the sentence into the encoder model to learn a rich representation to improve the classification accuracy~\cite{DBLP:conf/emnlp/XuMLCPJ15,DBLP:conf/acl/MiwaB16,DBLP:conf/emnlp/Zhang0M18,DBLP:conf/acl/GuoZL19}. While effective, these methods are limited to the relation classification task with given entities.





%Extracting relational facts from the raw text is one of the most important tasks in natural language processing.
%In the earlier relation extraction (RC) task, the goal is to classify the relation between two given entities into one of the pre-defined relations. Most researchers adopted sequence based models and attention mechanisms to encode each word sentence and distill a vector representation, which is then passed to a classifier~\cite{DBLP:conf/paclic/ZhangZHY15,DBLP:conf/coling/ShenH16,DBLP:conf/acl/WangCML16}.
%Some other studies also incorporate the dependency grammar information of the sentence into the encoder model to achieve a better representation and classification accuracy~\cite{DBLP:conf/emnlp/XuMLCPJ15,DBLP:conf/acl/MiwaB16,DBLP:conf/emnlp/Zhang0M18,DBLP:conf/acl/GuoZL19}.
%These methods, while effective, are limited to the relation extraction task with given entities.


% The natural solution is to address this task by two subtasks: firstly extracting all entities in the sentence, then classifying the relation between all entity pairs with traditional RC approaches.
% Extracting entities in a sentence, i.e. named entity recognition (NER), is a well-studied problem. Existing works include~\cite{DBLP:conf/acl/XuJW17,DBLP:conf/acl/GregoricBC18,DBLP:conf/acl/LiuYL19,DBLP:conf/acl/AroraTTKY19}.
% Many studies have adopted NER and RC approaches in a pipelined manner to solve the relation extraction without given entities~\cite{DBLP:journals/jmlr/ZelenkoAR03,DBLP:conf/acl/ZhouSZZ05,DBLP:conf/acl/ChanR11}. In addition multi-task learning approaches, including~\cite{DBLP:conf/aaai/WuH16,DBLP:conf/acl/AugensteinS17,DBLP:conf/emnlp/LiL17,DBLP:conf/emnlp/LuanHOH18,DBLP:conf/acl/LiZS19} can also be applied to solve the NER and RC tasks simultaneously. 
% However, the pipeline based methods may result in error propagation through the pipeline, which hurts the final relation extraction performance.
%

%\textcolor{red}{jointly extracting entities and relation~\cite{DBLP:conf/acl/ZhengWBHZX17,DBLP:conf/emnlp/Zhang0M18,zeng-etal-2019-learning,DBLP:conf/aaai/TakanobuZLH19,DBLP:conf/aaai/DaiXLDSW19}}

%It fails to handle cases where multiple relations exist between two entities.

In contrast to the previous methods~\cite{DBLP:conf/paclic/ZhangZHY15} where entities are assumed to be given in the text, a joint extraction of entities and relations is more practical~\cite{DBLP:conf/acl/ZhengWBHZX17,DBLP:conf/emnlp/Zhang0M18,zeng-etal-2019-learning,DBLP:conf/aaai/TakanobuZLH19,DBLP:conf/aaai/DaiXLDSW19}. Previous neural methods proposed for jointly extracting entities and relations can generally be categorized into three classes. The first class approach the joint extraction task as a sequence labeling problem~\cite{DBLP:conf/acl/ZhengWBHZX17,DBLP:conf/aaai/DaiXLDSW19,DBLP:conf/aaai/TakanobuZLH19,DBLP:journals/corr/abs-1909-04273}. \cite{DBLP:conf/acl/ZhengWBHZX17} is one of the first works which proposed a tagging strategy, thus, transferring the joint extraction task into a sequence labeling problem, where the label of relation and entity type are shared in a common space. However, this method has the fundamental weakness of addressing the overlapping problem of relational facts in the text. To meet it, \cite{DBLP:conf/aaai/DaiXLDSW19} proposed a position-attentive tagging scheme to solve the overlapping problem. Meanwhile, \cite{DBLP:conf/aaai/TakanobuZLH19} adopts a decomposition framework, where the joint extraction task is decomposed into a high-level relation detection task and a low-level task for entity extraction to resolve the overlapping problem. Other works~\cite{DBLP:journals/corr/abs-1909-04273} approach the problem by decomposing the joint extraction task into two sequence labeling sub-tasks, where one attempts to detect the subject of the relational fact, and the other detects its object with respect to the relation type

%\textcolor{red}{To solve the the problem of the sequence labeling problem, \cite{DBLP:conf/aaai/DaiXLDSW19} propose a position-attentive tagging scheme to solve the overlapping problem. \cite{DBLP:conf/aaai/TakanobuZLH19} address this overlapping problem from another point. They decomposing the relation extraction task into a high-level relation detection task, and a low-level task for entity extraction. They firstly identity a relation existing in the sentence, and then extracts the entities based on the detected relation. \cite{DBLP:journals/corr/abs-1909-04273} also propose to decompose the relation extraction task into two sequence labeling sub-taks. One is the subjection detection task, and another is the object detection task. They first detect a subject of the relational triple, and then detect its object which is associated with the relation type.}

The second class of works use a sequence-to-sequence (seq2seq) approach to address the problem~\cite{DBLP:conf/emnlp/Zhang0M18,zeng-etal-2019-learning}. Seq2seq models directly extract relational facts from the sentence by decoding the first entity, second entity, and relation in that order. \cite{DBLP:conf/emnlp/Zhang0M18} employs a seq2seq model to extract relational facts. But, their approach is limited to extracting a predefined number of relational facts from the text. In extracting relational triples, the order of extraction is key to identify the relational facts, as one relational triple may influence the truth value of another~\cite{zeng-etal-2019-learning}. As such, \cite{zeng-etal-2019-learning} proposed a seq2seq approach which utilizes a reinforcement learning model to learn the order of extracting the relational triples. Although effective, the proposed seq2seq models~\cite{DBLP:conf/emnlp/Zhang0M18,zeng-etal-2019-learning} only decode a single word for an entity. 

%A recent seq2seq-based model~\cite{zeng2019copymtl} attempts to solve this problem by integrating an ER model in its architecture to extract the entities multi-tokens.

%\cite{zeng-etal-2019-learning} extend a seq2seq model by adopting a \textcolor{red}{reinforcement learning model} to learn the order of extracting the relational triples. 

%Although effective, most \textcolor{red}{seq2seq models~\cite{}} only decode a single word for an entity. Thus, these methods cannot extract entities with multi-tokens. \textcolor{red}{To address this limitation of seq2seq task, \cite{zeng2019copymtl} propose to introduce a ER module to extract the entities.}



%\textcolor{red}{Previous neural models for jointly extracting entities can be divided into two class. One class is to treat the joint problem as a sequence labeling problem. \cite{DBLP:conf/acl/ZhengWBHZX17} is the first to propose a tagging strategy, transferring the joint task into a sequence labeling problem. However, it can not address the overlapping problem. }

%\textcolor{red}{Another is the seq2seq  models~\cite{DBLP:conf/emnlp/Zhang0M18,zeng-etal-2019-learning}. The seq2seq models directly extract relational triples from the sentence. They firstly decode first entity, then the second entity and finally the relation. These seq2seq models only decode a single word for an entity, thus can not extract the completed multi-token entities. Some seq2seq models also introduce reinforce learning method to model the order of extracting the relational triples~\cite{zeng-etal-2019-learning}}




%A more challenging task is to extract all relational facts from an arbitrary sentence which are not accompanied by marked entities. Recently, deep neural network based models are exploited to jointly learn ER and RC tasks. In \cite{DBLP:conf/acl/ZhengWBHZX17}, authors propose a tagging strategy to transfer the joint task into a sequence prediction problem, where the label of relation and entity type are shared in a common space. This joint model is capable of extracting entities and relations simultaneously. However, it fails to handle the case where more than one relations exist between two entities. In \cite{DBLP:conf/emnlp/Zhang0M18}, authors propose an end-to-end sequence-to-sequence model which detects a relational triple by firstly decoding the relation, and further decoding the two entities of the relation. However, the number of relational triples that can be extracted in a sentence is limited to a predefined constant. This model cannot extract entities containing multiple words as well.

%\textcolor{red}{jointly extracting entities and relation using MTL~\cite{zeng2019copymtl,DBLP:conf/acl/MiwaB16,DBLP:conf/acl/FuLM19}}

The third class design a multi-task learning architecture to extract relational facts~\cite{DBLP:conf/acl/MiwaB16,DBLP:conf/acl/FuLM19,zeng2019copymtl}. \cite{DBLP:conf/acl/MiwaB16} is one of the first works to extract relational facts using an MTL framework. Following this work, some recent MTL-based methods have been proposed~\cite{DBLP:conf/acl/FuLM19,zeng2019copymtl}. Particularly, \cite{zeng2019copymtl} proposed an MTL architecture which comprises of an ER model to extract entities with multi-tokens, and a seq2seq model to identify and extract relational facts. Their approach solves the entity extraction problem faced by models which are solely seq2seq based. \cite{DBLP:conf/acl/FuLM19} also exploits a Bidirectional Recurrent Neural Network (Bi-RNN) and Graph Convolutional Network (GCN) to extract common features of the ER and RC tasks, which are further fed into two independent classifiers for ER and RC predictions.  Despite the substantial efforts and great successes in the design of these MTL-based methods, these methods follow the conventional multi-task learning approach~\cite{DBLP:conf/icml/CollobertW08}. Thus, they only learn implicit interactions between the ER and RC tasks. 

%\textcolor{red}{\cite{DBLP:conf/acl/MiwaB16} is one of the works to solve the relation extraction task using a MTL framework. They learn shared representations which are passed to the task-specific channels for prediction. Similarly, \cite{DBLP:conf/acl/FuLM19} feed the shared representations into two separately classifiers for ER and RC prediction. \cite{zeng2019copymtl} is discussed above. They extend a seq2seq model by introducing a ER module to extract all entities in the sentence. Their model is a MTL framework.}

%It is worth noting that the above mentioned works seldom consider the implicit constraint and connections between ER and RE. Multi-task learning techniques are introduced to implicitly model the interaction between ER and RE. In \cite{DBLP:conf/acl/FuLM19}, authors follow the generalized MTL framework and exploit Bi-RNN and GCN to extract both sequential and regional dependency word features of the sentence. The shared features are then fed into two independent classifiers for RC and ER respectively. A

Modelling explicit interactions between multiple tasks in an MTL architecture have been explored to improve predictions in several domains ~\cite{DBLP:conf/acl/HeLND19,DBLP:conf/aaai/Zhao0ZW19,DBLP:conf/emnlp/DankersRLS19,DBLP:conf/emnlp/LanWWNW17,DBLP:conf/aaai/LiuFDQC19,DBLP:conf/ijcai/LiuQH16}. For instance, \cite{DBLP:conf/ijcai/LiuQH16} explore a message passing mechanism for text classification. \cite{DBLP:conf/aaai/LiuFDQC19} extends \cite{DBLP:conf/ijcai/LiuQH16} by proposing a generalized MTL model with a message passing mechanism to dynamically learn interactions between multiple tasks. Other methods have proposed gating mechanisms to learn the explicit interactions for sentence-level regression~\cite{DBLP:conf/emnlp/DankersRLS19} and implicit discourse relation recognition~\cite{DBLP:conf/emnlp/LanWWNW17}. Explicit interactions have also been modelled in a multi-task learning architecture for medical named entity recognition and normalization~\cite{DBLP:conf/emnlp/DankersRLS19} and aspect-based sentiment classification~\cite{DBLP:conf/acl/HeLND19}. As mentioned in Section~\ref{introduction}, it is difficult to effectively learn the correlations between the ER and the RC tasks. To this end, we follow some of the ideas from other domains to dynamically learn the interactions between the two tasks, refining the classifiers of the tasks. To the best of our knowledge, this is the first work to model explicit interactions in a multi-task learning architecture for the joint extraction of entities and relations in text. 

% \textcolor{red}{MTL with explicit interactions~\cite{DBLP:conf/acl/HeLND19,DBLP:conf/aaai/Zhao0ZW19,DBLP:conf/emnlp/DankersRLS19,DBLP:conf/emnlp/LanWWNW17,DBLP:conf/aaai/LiuFDQC19,DBLP:conf/ijcai/LiuQH16}}

% \textcolor{red}{The interaction MTL works can be divided into two classes. One class can be called low-level interaction which does not consider the output of different sub-tasks. This kind of models learn task-specific features separately for the tasks. Then they employ message passing mechanism~\cite{DBLP:conf/aaai/LiuFDQC19,DBLP:conf/ijcai/LiuQH16} or the gate mechanism~\cite{DBLP:conf/emnlp/DankersRLS19,DBLP:conf/emnlp/LanWWNW17} to model the interaction between the task-specific features.} 

% \textcolor{red}{Recently, Another class is the high-level interaction which considers the output of different sub-tasks~\cite{DBLP:conf/aaai/Zhao0ZW19,DBLP:conf/acl/HeLND19}. However, they use simple linear transformation which takes in the outputs of different tasks to learn a interaction feature. The interaction feature is used to update the shared hidden states. The interaction in their models is ran for only once, and a simple linear transformation can not sufficiently model the interaction.}


% \textcolor{red}{\cite{DBLP:conf/acl/HeLND19} proposed an interactive multi-task learning network for jointly extracting aspects and classifying their sentiment. Both sub-tasks are regarded as a sequence prediction problem which is not the same as our joint NER and RC model. In addition, a linear transformation is exploited for the interaction of the outputs of sub-tasks is not sufficient to model the interaction between models.}




% As discussed in the Introduction section, the explicit correlation is also a potential constraint to improve the learning of both the NER and RC model.



% In this paper, we not only proposed to consider the constraint by learning the ``alignment'' information of NER and RC on each word, but also introduce the recurrent interaction network to sufficiently capture the correlation of two tasks. The experiment results show that the extraction of entities and relations is refined in the recurrent interaction process.
% The most related work \cite{DBLP:conf/acl/FuLM19} considered the interaction between entities and relations by applying a 2nd-phase entity and relation prediction after the 1st-phase prediction. The model exploit bi-RNN and GCN to extract both sequential and regional dependency word features of the sentence. Based on the
% same feature encodings, both relations for each word pair and the entities for all words are predicted.
% Based on the relation prediction results, they further applied a 2nd-phase GCN on the detected entity pairs for each relation type. After relation weighted propagations over GCN, it is supposed to extract more sufficient features for each word. However, their model follows the generalized MTL framework. The shared features encoded by bi-RNN and GCN are fed into two independent classifiers for RC and NER respectively. The implicit constraints between the two task are not considered and the interaction of the two tasks is not explicitly modeled.

% \begin{figure*}[htbp]
% 	\centering
% 	\scalebox{1.}{\input{our_model.tex}}
% 	\caption{Overview of RIN. The $f_r$ extracts relation-specific feature ${\tilde H}$ and $f_g$ extracts entity-specific feature ${\bar H}$ from the sentence embedding $H$. The $C_r$ is relation extraction model and the $C_g$ is the entity recognition model. INT encodes the interaction information between two sub-tasks. }
% 	\label{fig:our_model}
% \end{figure*} 

\begin{figure*}[htbp]
	\centering
	\renewcommand\tabcolsep{1.5pt}
	\begin{tabular}{c c c}
	\scalebox{0.65}{\input{our_model.tex}}
	&
	\scalebox{0.65}{\input{Cg.tex}}&\scalebox{0.65}{\input{Cr.tex}}
	\\
	(A) & (B) & (C)
	\end{tabular}
	\caption{(A) Overview of RIN. (B) The Cg module for entity recognition. (C) The Cr module for relation classification. Take a sentence with three words as example. Assume representations of the sentence $H=\{h_1, h_2, h_3\}$ are given. The bias terms are omitted. For the Cr module, we only take the $w_1$ as example. It predicts the relations of all the word pairs $<w1, \cdot>$. $+$ donates the concatenate operation in (C) and donates an summation in (A), $*$ donates the 
matrix multiplication, $\phi$ donates the relu activation function, $\sigma$ donates the sigmoid function.}
	\label{fig:our_model}
\end{figure*}
